SR-LLM: Rethinking the Structured Representation in Large Language Model

Structured representations, exemplified by Abstract Meaning Representation (AMR), have long been pivotal in computational linguistics. However, their role remains ambiguous in the Large Language Models (LLMs) era. Initial attempts to integrate structured representation into LLMs via a zero-shot setting yielded inferior performance. We hypothesize that such a decline stems from the structure information being passed into LLMs in a code format unfamiliar to LLMs' training corpora. Consequently, we propose SR-LLM, an innovative framework with two settings to explore a superior way of integrating structured representation with LLMs from training-free and training-dependent perspectives. The former integrates structural information through natural language descriptions in LLM prompts, whereas its counterpart augments the model's inference capability through fine-tuning on linguistically described structured representations. Performance improvements were observed in widely downstream datasets, with particularly notable gains of 3.17% and 12.38% in PAWS. To the best of our knowledge, this work represents the pioneering demonstration that leveraging structural representations can substantially enhance LLMs' inference capability. We hope that our work sheds light and encourages future research to enhance the reasoning and interoperability of LLMs by structure data.

==> tex/acknowledgements.tex <==
\subsubsection*{Acknowledgments}
Use unnumbered third level headings for the acknowledgments. All
acknowledgments, including those to funding agencies, go at the end of the paper.

==> tex/background.tex <==
\section{Background}
The structure representations of AMR, PST, and FOL each have their unique advantages and applications in semantic abstraction, syntactic parsing, and logical reasoning, respectively. Abstract Meaning Representations (AMRs) are rooted, labeled graph structures designed to abstract away from syntactic nuances, providing concise and semantically rich representations ~\citep{banarescu2013abstract}. Phrase Syntax Trees (PSTs) are hierarchical tree structures grounded in Chomsky’s theory of generative grammar, commonly used to represent the syntactic organization of sentences, emphasizing the dependency between words~\citep{chomsky2014aspects}. First-Order Logics (FOLs) are symbolic logic systems that articulate objects, their relationships, and properties, making them essential tools in formal logic and logical reasoning~\citep{enderton2001mathematical, BARWISE19775}. 

